Dual Debiasing: Remove Stereotypes and Keep Factual Gender for Fair Language Modeling and Translation

Mitigation of biases, such as language models' reliance on gender stereotypes, is a crucial endeavor required for the creation of reliable and useful language technology. The crucial aspect of debiasing is to ensure that the models preserve their versatile capabilities, including their ability to solve language tasks and equitably represent various genders. To address this issue, we introduce a streamlined Dual Dabiasing Algorithm through Model Adaptation (2DAMA). Novel Dual Debiasing enables robust reduction of stereotypical bias while preserving desired factual gender information encoded by language models. We show that 2DAMA effectively reduces gender bias in English and is one of the first approaches facilitating the mitigation of stereotypical tendencies in translation. The proposed method's key advantage is the preservation of factual gender cues, which are useful in a wide range of natural language processing tasks.

==> figures/OLD_figure_one.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/Bias_Factual_Comaprison.png}
    \caption{Dual character of gender signals encoded in language models:
    \textcolor{schema_blue}{stereotypical} cues are shown on the left, and \textcolor{schema_orange}{factual} gender cues are shown on the right-hand side.}
    \label{fig:figure-one}
\end{figure}

==> tables/2dama_translation_L12.tex <==
\begin{table*}[!th]
\centering
\begin{adjustbox}{max width=\linewidth}
\small
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\multirow{2}{*}{Language} & \multirow{2}{*}{} & \multicolumn{2}{c}{Translation to English} & \multicolumn{2}{c}{Translation from English} & \multicolumn{2}{c}{WinoMT} & \multicolumn{2}{c}{BUG} \\ \cmidrule(r){3-4} \cmidrule(rl){5-6} \cmidrule(rl){7-8} \cmidrule(l){9-10}   
 &  & $\uparrow$ comet & $\uparrow$ chrf & $\uparrow$ comet & $\uparrow$ chrf & $\downarrow$ $\Delta S$ & $\downarrow$ $\Delta G$ & $\downarrow$ $\Delta S$ & $\downarrow$ $\Delta G$ \\ \midrule
\multirow{4}{*}{German} & ALMAR 13B & 85.0 & 57.0 & 86.7 & 58.1 & 30.5 & 3.7 & 7.8 & 32.5 \\
 & DAMA+LEACE & 85.3 & 55.4 & 84.7 & 54.3 & 7.9 & 2.2 & 6.6 & 30.6 \\
 & 2DAMA ($t=0.05$) & 85.1 & 54.8 & 84.2 & 53.6 & 14.4 & 1.4 & 4.5 & 27.2 \\
 & 2DAMA ($t=1.00$) & 85.4 & 55.4 & 84.9 & 54.4 & 13.5 & -17.4 & 4.7 & 26.8 \\ \midrule
\multirow{4}{*}{Czech} & ALMAR 13B & 89.7 & 53.8 & 89.7 & 53.8 & 26.3 & 2.1 & 11.7 & 9.2 \\
 & DAMA+LEACE & 88.5 & 49.5 & 88.5 & 49.5 & 19.9 & 19.1 & 9.6 & 18.1 \\
 & 2DAMA ($t=0.05$) & 88.3 & 49.1 & 88.3 & 49.1 & 17.2 & 15.7 & 7.2 & 12.9 \\
 & 2DAMA ($t=1.00$) & 88.7 & 50.2 & 88.7 & 50.2 & 24.7 & 8.7 & 11.4 & 13.1 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Evaluation of gender bias and quality of translation.
In all the methods, ALMA-R was used as the base model.
In each setting, except the original, adaptations were applied to 12 mid-upper feed-forward layers. 
Translation quality was evaluated on the WMT-22 dataset. 
}
\label{tab:2dama-translation-12l}
\end{table*}

==> tables/OLD_2dama_bias.tex <==
\begin{table}[!th]
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lccccc@{}}
\toprule
           & \multicolumn{3}{c}{Bias in LM}                           & \multicolumn{2}{c}{WinoBias}                      \\ \cmidrule(rl){2-4} \cmidrule(l){5-6}
           & $\downarrow$ $a_s$ & $\uparrow$ $a_f$ & $\downarrow$ $b$ & $\downarrow$ $\Delta S$ & $\downarrow$ $\Delta G$ \\ \midrule
LLaMA2 7B  & 0.234 & 0.311 & 0.090 & 33.63\% & 7.28\% \\
DAMA       & 0.144 & 0.205 & 0.032 & 27.31\% & 6.78\% \\
DAMA+LEACE & 0.118 & 0.171 & 0.028 & 22.90\% & 5.41\% \\
2DAMA      & 0.128 & 0.187 & 0.042 & 22.90\% & 5.67\% \\ \midrule
LLaMA2 13B & 0.244 & 0.322 & 0.097 & 35.01\% & 0.29\% \\
DAMA       & 0.099 & 0.160 & 0.030 & 26.44\% & 2.35\% \\
DAMA+LEACE & 0.098 & 0.159 & 0.026 & 26.45\% & 2.35\% \\
2DAMA      & 0.119 & 0.206 & 0.023 & 26.95\% & 1.85\% \\ \midrule
ALMA-R 13B & 0.267 & 0.359 & 0.104 & 39.70\% & 1.73\% \\
DAMA+LEACE & 0.124 & 0.203 & 0.024 & 35.68\% & 5.54\% \\
2DAMA      & 0.153 & 0.261 & 0.044 & 33.53\% & 6.19\% \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Bias evaluation for the \llama{} family models, and their adaptation with different debiasing algorithms (\dama{}, \dama{} with \leace{}, and \ddama{}).
The debiasing adaptation was performed with \ddama{} on 11 mid-upper layers with the bias-to-feature threshold set to $t=0.05$ in \ddama{}.
}
\label{tab:2dama-bias}
\end{table}

==> tables/OLD_2dama_general.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lccc@{}}
\toprule
           & LM               & \multicolumn{2}{c}{ARC}                 \\ \cmidrule(l){3-4} 
           & $\downarrow$ ppl & $\uparrow$ acc (C) & $\uparrow$ acc (E) \\ \midrule
LLaMA2 7B  & 21.28            & 70.2\%             & 42.5\%             \\
DAMA       & 21.51            & 69.8\%             & 42.8\%             \\
DAMA+LEACE & 23.81            & 68.3\%             & 41.2\%             \\
2DAMA      & 23.66            & 67.5\%             & 42.0\%             \\ \midrule
LLaMA2 13B & 19.68            & 72.6\%             & 46.8\%             \\
DAMA       & 18.94            & 71.6\%             & 45.0\%             \\
DAMA+LEACE & 19.67            & 71.3\%             & 46.4\%             \\
2DAMA      & 19.90            & 71.2\%             & 46.1\%             \\ \midrule
ALMA-R 13B & 26.90            & 68.9\%             & 44.0\%             \\
DAMA+LEACE & 19.44            & 68.1\%             & 44.0\%             \\
2DAMA      & 19.04            & 67.6\%             & 43.6\%             \\ \bottomrule
\end{tabular}
\caption{General performance in language modeling and question answering of \llama{} family models, and their adaptation with different debiasing algorithms (\dama{}, \dama{} with \leace{}, and \ddama{}).
The hyperparameters are the same as in Table~\ref{tab:2dama-bias}}
\label{tab:2dama-general}
\end{table}

==> tables/dama_leace_bias.tex <==
\begin{table}[!th]
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
            & \multicolumn{2}{c}{Bias in LM}                     & \multicolumn{2}{c}{WinoBias}     & \multicolumn{2}{c}{StereoSet} \\\cmidrule(r){2-3}\cmidrule(lr){4-5}\cmidrule(l){6-7}
            & $\downarrow$ $a_s$ & $\downarrow$ $b$    &  $\downarrow$ $\Delta S$ & $\downarrow$ $\Delta G$ & $\downarrow$ ss & $\uparrow$ ICAT  \\ \midrule
LLaMA 7B  & 0.235        & 0.072        & 40.3\%       & 3.0\%       & 71.9       & 53.7      \\
+ DAMA    & -0.005       & -0.006       & 32.5\%       & 2.4\%       & 68.4       & 60.5       \\
+ DAMA-L  & \underline{-0.019} & \underline{-0.002} & \underline{25.5\%} & \underline{1.6\%} & \underline{68.0} & \underline{61.0} \\ \midrule
LLaMA 13B & 0.270        & 0.068        & 35.7\%       & -1.5\%      & 71.8       & 53.7       \\
+ DAMA    & 0.115        & 0.042        & 29.5\%       & \underline{1.2\%} & 70.3       & 55.9       \\
+ DAMA-L  & \underline{0.104}  & \underline{0.039}  & \underline{26.3\%} & 2.2\%       & \underline{69.6} & \underline{57.2} \\ \bottomrule 

\end{tabular}
\end{adjustbox}
\caption{Bias evaluation for the LLaMA 7B and 13B models, and their adaptation with DAMA and DAMA-L(EACE).
We underline the best value in each column.
}
\label{tab:dama-leace-bias}
\end{table}

==> tables/dama_leace_general.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}lccccc@{}}
\toprule
            & LM   & \multicolumn{2}{c}{ARC} \\ \cmidrule(l){3-4}
            & $\downarrow$ PPL  & $\uparrow$ acc (C)     & $\uparrow$ ACC (E) \\ \midrule
LLaMA 7B  & 26.1 & 69.2\% & 42.7\% \\
+ DAMA    & 29.3 & 68.7\% & 42.7\% \\
+ DAMA-L  & 29.4 & 67.4\% & 42.2\% \\ \midrule
LLaMA 13B & 19.8 & 71.2\% & 44.5\% \\
+ DAMA    & 20.2 & 70.7\% & 43.3\% \\
+ DAMA-L  & 21.1 & 70.5\% & 43.8\% \\ \bottomrule
\end{tabular}
\caption{General performance evaluation for the LLaMA 7B and 13B models, and their adaptation with DAMA and DAMA-L(EACE).}
\label{tab:dama-leace-general}
\end{table}

==> tables/translation_bias.tex <==
\begin{table}[!tb]
\tiny
\centering
\begin{tabular}{@{}llrrrrrrrrr@{}}
\toprule
  & \multicolumn{3}{c}{\textbf{acc}} & \multicolumn{3}{c}{\textbf{$\Delta$ G}} & \multicolumn{3}{c}{\textbf{$\Delta$ S}} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(l){8-10}
  & \multicolumn{1}{c}{cs} & \multicolumn{1}{c}{de} & \multicolumn{1}{c}{ru} & \multicolumn{1}{c}{cs} & \multicolumn{1}{c}{de} & \multicolumn{1}{c}{ru} & \multicolumn{1}{c}{cs} & \multicolumn{1}{c}{de} & \multicolumn{1}{c}{ru} \\ \midrule
ALMA-R & 77.6 & 65.6 & 44.6 & 2.4 & 3.0 & 25.4 & 25.9 & 29.6 & 10.4 \\
+DAMA & 75.7 & 64.5 & 45.2 & 4.0 & 4.2 & 24.4 & 24.2 & 31.0 & 7.4 \\
+M. DAMA & 53.1 & 56.7 & 41.8 & 23.3 & 19.6 & 32.7 & 19.1 & 22.8 & 7.4 \\ \bottomrule
\end{tabular}
\caption{WinoMT Results}
\label{tab:wino-mt}
\end{table}

==> tables/translation_performance.tex <==
\begin{table*}[!tb]
\small
\centering
\begin{tabular}{@{}llcccccccccc@{}}
\toprule
 &  \multicolumn{2}{c}{\textbf{en-cs}} & \multicolumn{2}{c}{\textbf{en-de}} & \multicolumn{2}{c}{\textbf{en-is}} & \multicolumn{2}{c}{\textbf{en-ru}} & \multicolumn{2}{c}{\textbf{en-zh}} \\ 
 & BLEU & chrf & BLEU & chrf & BLEU & chrf & BLEU & chrf & BLEU & chrf \\
 \midrule
 ALMA-R & 25.93 & 53.71 & 28.18 & 58.06 & 21.00 & 52.44 & 24.43 & 52.20 & 16.29 & 33.58 \\
 +DAMA & 22.88 & 51.65 & 26.56 & 56.85 & 18.72 & 50.77 & 23.81 & 51.90 & 15.24 & 32.34 \\
+M DAMA & 19.64 & 49.12 & 25.90 & 56.73 & 18.43 & 50.70 & 23.03 & 51.51 & 14.12 & 32.52 \\ \midrule
 & \multicolumn{2}{c}{\textbf{cs-en}} & \multicolumn{2}{c}{\textbf{de-en}} & \multicolumn{2}{c}{\textbf{is-en}} & \multicolumn{2}{c}{\textbf{ru-en}} & \multicolumn{2}{c}{\textbf{zh-en}} \\
 & BLEU & chrf & BLEU & chrf & BLEU & chrf & BLEU & chrf & BLEU & chrf \\ \midrule
ALMA-R & 68.55 & 45.39 & 31.03 & 56.50 & 40.28 & 62.77 & 39.85 & 65.73 & 22.88 & 52.22 \\
+DAMA & 67.68 & 43.32 & 31.15 & 56.81 & 39.65 & 62.41 & 38.55 & 65.04 & 21.89 & 51.18 \\
+M DAMA & 67.71 & 43.34 & 30.76 & 56.42 & 39.48 & 62.66 & 38.75 & 65.24 & 22.27 & 51.32 \\ \bottomrule
\end{tabular}
\caption{WMT-22 Results}
\label{tab:wmt-22}
\end{table*}

==> tables/xlingual_chrf.tex <==
\begin{table}[!h]
\centering
\small
\begin{tabular}{@{}cccc@{}}
\toprule
Prompt Lang. $\downarrow$ & German & Czech & Russian \\ \midrule
$\emptyset$   & 57.4   & 52.3  & 52.1    \\
English       & 57.0   & 51.2  & 51.6    \\
German        & 54.8   & 50.6  & 51.1    \\
Czech         & 57.5   & 49.9  & 51.8    \\
All Above     & 55.5   & 48.1  & 51.1    \\ \bottomrule
\end{tabular}
\caption{The values of chrf on WMT-22.
The evaluation target language is shown at the top of each column.
Each row corresponds to a set of languages for which prompts were used in model adaptation.
The debiasing adaptation was performed with \ddama{} on 11 mid-upper layers with the bias-to-stereotype ratio set to $t=0.05$.
}
\label{tab:xlingual-chrf}
\end{table}

==> tables/xlingual_deltaG.tex <==
\begin{table}[!h]
\centering
\small
\begin{tabular}{@{}cccc@{}}
\toprule
Prompt Lang. $\downarrow$ & German & Czech & Russian \\ \midrule
$\emptyset$   & 3.7    & 2.1   & 25.7    \\
English       & 11.1   & 7.9   & 31.4    \\
German        & 3.3    & 21.6  & 31.3    \\
Czech         & 6.2    & 14.6  & 32.0     \\
All Above     & 8.1    & 23.2  & 33.4    \\ \bottomrule
\end{tabular}
\caption{Representational bias ($\Delta G$) in the WinoMT challenge-set.
The evaluation target language is shown at the top of each column.
Each row corresponds to a set of languages for which prompts were used in model adaptation.
The debiasing adaptation was performed with \ddama{} on 11 mid-upper layers with the bias-to-feature ratio set to $t=0.05$.
}
\label{tab:xlingual-deltaG}
\end{table}

==> tables/xlingual_deltaS.tex <==
\begin{table}[!h]
\centering
\small
\begin{tabular}{@{}cccc@{}}
\toprule
Prompt Lang. $\downarrow$ & German & Czech & Russian \\ \midrule
$\emptyset$    & 30.5   & 26.3  & 10.2    \\
English        & 28.1   & 22.9  & 8.5     \\
German         & 22.1   & 17.4  & 3.0     \\
Czech          & 26.5   & 18.0  & 4.7     \\
All Above      & 30.0   & 17.8  & 1.1     \\ \bottomrule
\end{tabular}
\caption{The values of $\Delta S$ in the WinoMT challenge-set.
The evaluation target language is shown at the top of each column.
Each row corresponds to a set of languages for which prompts were used in model adaptation.
The debiasing adaptation was performed with \ddama{} on 11 mid-upper layers with the bias-to-stereotype ratio set to $t=0.05$.
}
\label{tab:xlingual-deltaS}
\end{table}

==> tables/xlingual_deltaS_L12.tex <==
\begin{table}[!h]
\centering
\small
\begin{tabular}{@{}cccc@{}}
\toprule
Prompt Lang. $\downarrow$ & German & Czech & Russian \\ \midrule
$\emptyset$    & 30.5   & 26.3  & 10.2    \\
English        & 28.5   & 21.2  & 7.0     \\
German         & 14.4   & 15.1  & 4.0     \\
Czech          & 24.3   & 17.2  & 3.9     \\
All Above      & 24.0   & 18.7  & 1.3     \\ \bottomrule
\end{tabular}
\caption{Stereotypical bias ($\Delta S$) in the WinoMT challenge-set.
The evaluation target language is shown at the top of each column.
Each row corresponds to a set of languages for which prompts were used in model adaptation.
The debiasing adaptation was performed with \ddama{} on 12 mid-upper layers with the bias-to-feature ratio set to $t=0.05$.
}
\label{tab:xlingual-deltaS-12l}
\end{table}
